Sample Efficient Learning of Path Following and Obstacle Avoidance Behavior for Quadrotors

In this paper we propose an algorithm for the training of neural network control policies for quadrotors. The learned control policy computes control commands directly from sensor inputs and is hence computationally efficient. An imitation learning algorithm produces a policy that reproduces the behavior of a path following control algorithm with collision avoidance. Due to the generalization ability of neural networks, the resulting policy performs local collision avoidance of unseen obstacles while following a global reference path. The algorithm uses a time-free model predictive path-following controller as a supervisor. The controller generates demonstrations by following few example paths. This enables an easy to implement learning algorithm that is robust to errors of the model used in the model predictive controller. The policy is trained on the real quadrotor, which requires collision-free exploration around the example path. An adapted version of the supervisor is used to enable exploration. Thus, the policy can be trained from a relatively small number of examples on the real quadrotor, making the training sample efficient.

==> sec/031_implementation.tex <==
\section{Implementation}










\subsection{Example Paths}\label{sec:mot_prim}

To learn a certain skill, like path tracking or collision avoidance, the policy needs several examples of this behavior. Currently, we only use two skills with examples produced via a simple heuristics (Fig.~\ref{fig:setpointChange}). First, examples of the quadrotor approaching the global path at an angle of $45^o$ are created from different starting positions. Second, we provide examples for obstacle avoidance with the maneuver always starting $3~m$ from the obstacle and passing it at a distance of $1.5~m$. Importantly, these paths do not need to take the physical model of the robot into account (because they are time-free) and could simply be drawn by a user. The spline is a natural cubic spline that passes through control points, which can be obtained by sampling or direct positioning of control points.

\subsection{Global Path Following}\label{sec:global_path}

The global guidance $\globalPath$ coarsely specifies the quadrotor motion but needs not be aware of obstacles. At training and test time we define a setpoint which is moving along the path with constant velocity. For training and testing we compute the distance of the position measurement obtained from odometry and this setpoint in the quadrotor frame:
\begin{equation}
d = (\vp_{odom} - \vp_{setpoint}) R(\phi) .
\end{equation}
Where $R(\phi)$ is a rotation matrix around $z$. The angle $\phi$ is calculated from the global path tangent (see Fig.~\ref{fig:physics_contour}). The vector $d$ is used as input to the policy. The policy controls translation of the quadrotor, while the yaw angle is controlled separately with a simple PD controller to ensure that the quadrotor always faces the direction of the global path (the distance sensor points in this direction). This parametrization allows for training on straight guidance splines, while at test time this can be applied to arbitrary splines (Fig.~\ref{fig:train_test}).


\subsection{Neural network training}\label{sec:nn_train}
Training of the neural network is done in an iterative fashion using the TensorFlow deep-learning library, initializing each iteration from the previous solution. We use the ADAM optimization algorithm. The network architecture consists of a fully connected network with two hidden layers using soft ReLu neurons and linear neurons in the output layer.

